T2K ND280 Upgrade -- Technical Design Report

In this document, we present the Technical Design Report of the Upgrade of the T2K Near Detector ND280. The goal of this upgrade is to improve the Near Detector performance to measure the neutrino interaction rate and to constrain the neutrino interaction cross-sections so that the uncertainty in the number of predicted events at Super-Kamiokande is reduced to about 4%. This will allow to improve the physics reach of the T2K-II project. This goal is achieved by modifying the upstream part of the detector, adding a new highly granular scintillator detector (Super-FGD), two new TPCs (High-Angle TPC) and six TOF planes. Details about the detector concepts, design and construction methods are presented, as well as a first look at the test-beam data taken in Summer 2018. An update of the physics studies is also presented.

==> README <==
Preprint Collection:					(May 2013)
~~~~~~~~~~~~~~~~~~~~
This directory contains some packages written by Patrick W. Daly.  The
primary distribution site is:

http://www.mps.mpg.de/software/latex/localtex/localltx.html

I (Arash Esbati) mentioned balance.sty in comp.text.tex, was invited
to put in on CTAN, asked Patrick W. Daly for permission, wrote this
readme for your convenience and made a CTAN submission.


Legal stuff:
~~~~~~~~~~~~~~~~~~~~
The copyright holder of these packages is Patrick W. Daly.  They can be
redistributed and/or modified under the terms of the LaTeX Project Public
License Distributed from CTAN archives in directory
macros/latex/base/lppl.txt; either version 1 of the License, or any later
version.


Important note:
~~~~~~~~~~~~~~~~~~~~
Unfortunately, the author of these packages doesn't have the time for
further development, bug fixes, "wishes" etc.  Hence, they are provided
"as is".  If you run into problems, you are on your own.


Brief description:
~~~~~~~~~~~~~~~~~~~~
1. authblk.sty:   (version 1.3 from 2001/02/27)
   A LaTeX2e package to redefine the \author command to work as normal or
   to allow a footnote style of author/affiliation input.

2. balance.sty:   (version 4.3 from 1999/02/23)
   When writing a document with LaTeX two-column mode, the columns on the
   last page, or those before a \cleardoublepage command, will be of
   unequal height.  balance.sty solves this problem by modifying the output
   routines in two-column mode.

3. figcaps.sty:   (version 4.7 from 1999/02/23)
   This package allows the figure captions to be collected throughout the
   paper and printed on a separate page at the end.  The figures themselves
   will not appear in the text.  This is for purposes of a manuscript for
   submission.  Similarly, tables are not printed in the text, but are
   outputted at the end, after the figure captions.  This package may
   optionally be used with the longtable environment defined in the package
   of the same name.

4. fullpage.sty:  (version 1.1 from 1999/02/23)
   This package sets all 4 margins to be either 1 inch or 1.5 cm, and
   specifies the page style.

5. sublabel.sty   (version 4.5 from 1999/02/23)
   The macros in this package allow all counters to be subnumbered, as for
   example 4a, 4b, 4c, simply by bracketting the objects to be so numbered
   with appropriate on/off commands.  They will work with any user-defined
   counters too.

6. appendix.sty:  (version 2.2 from 2005/10/30)
   Adding this package redefines \appendix so that main counters for
   figures, tables, equations are subnumbered under the appendix.  The
   plate counter is also subnumbered.  A \noappendix command is included so
   that things like bibliographies may be called after the appendix with
   \section*.  This package is only useful with article documentclass for
   obvious reasons.

   N.B.: This package is not available on CTAN due to a name clash.  You 
   have to fetch it from the site mentioned above.


Installation:
~~~~~~~~~~~~~~~~~~~~
Just run LaTeX on (package).ins, which generates (package).sty.  If you
want the documentation as a dvi, run LaTeX on (package).dtx, otherwise use
the provided format.  Move the .sty-files to a directory where LaTeX looks
for the input files.  Update your file name database and you're done.
Check your local guide for more Information.


Happy TeXing!
      Arash Esbati


;; Local Variables:
;; mode: text
;; fill-column: 75
;; End:


==> ReadMe.tex <==
\chapter{Instructions}
Here some instructions which should help to ensure that the merging of the different chapters will be going smoothly. It would be desirable that for the figures, etc. not every chapter/author uses some very specific latex package but as much as possible common packages are used. 

\section{Outline}
For each chapter some suggestions for the outline of this specific chapter were made. In some cases very rudimentary and in other cases more elaborated. \\
These suggestions are based on previous TDRs for similar detectors but should be considered only suggestions. The editors of each chapter are invited to come up with other suggestions for their chapter.  

\section{Figure Names and Storage Directory}
Please give all figures names which simplify to identify to which chapter they belong! 
Examples for useful names for the case of the Target chapter are:
\begin{itemize}
\item Target\_XY.png
\item target\_XY.png
\item tar\_XY.png
\end{itemize}
All figures in the chapter should follow the same naming scheme. \\
Since arxiv has a problem with having figures in a subdirectory, please store them in the main directory! 

\section{Captions of Figures/Tables}
Please place the captions below the figures/tables. 

\section{Including Figures}
For the including of single plots, please use the following command: 
\begin{verbatim}
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.8\textwidth]{dummy_fig}
\caption{Example of single plot.}
\label{fig:single_fig}
\end{center}
\end{figure}
\end{verbatim}
The result is shown in Fig.~\ref{fig:single_fig}
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.8\textwidth]{dummy_fig}
\caption{Example of single plot.}
\label{fig:single_fig}
\end{center}
\end{figure}


\section{Multi-Figures/Tables}
For multi-figures/tables the packages subcaption should be used if possible. The base command for figures is:
\begin{verbatim}
\begin{figure}
\begin{subfigure}[b]{.5\linewidth}
\includegraphics[width=0.9\textwidth]{dummy_fig}
\centering
\caption{A subfigure}\label{fig:1a}
\end{subfigure}%
\begin{subfigure}[b]{.5\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{dummy_fig}
\caption{Another subfigure}\label{fig:1b}
\end{subfigure}
\caption{A figure}\label{fig:1}
\end{figure}
\end{verbatim}
The result is shown in Fig.~\ref{fig:1}

\begin{figure}
\begin{subfigure}[b]{.5\linewidth}
\includegraphics[width=0.9\textwidth]{dummy_fig}
\centering
\caption{A subfigure}\label{fig:1a}
\end{subfigure}%
\begin{subfigure}[b]{.5\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{dummy_fig}
\caption{Another subfigure}\label{fig:1b}
\end{subfigure}
\caption{A figure}\label{fig:1}
\end{figure}

\section{Labeling of/Referring to Figures and Tables}
To label and refer to figures or tables please use:
\begin{verbatim}
\label{fig:X} for a figure and \label{tab:Y} for a table. 
When referring to a figure or table please use: 
Fig.~\ref{fig:X} or Tab.~\ref{tab:Y}.
\end{verbatim}

\section{Bibliography}
For the bibliography Bibtex will be used. For each chapter there is a bib file with the same name as the latex file, e.g. TPC.tex and TPC.bib. All relevant references should be added to this file using, as far as possible, the official Bibtex entries e.g. from InspireHep so that references which might be used in different chapters are not appearing twice in the bibliography.  



==> Target_assembly.tex <==
\section{Detector assembly}
\subsection{Assembly of plastic cubes}



==> TestBeam-old.tex <==
-old\section{Test Beam}
\label{sec:testbeam}

During Summer 2018 a TPC has been assembled and operated at CERN using tagged beams from the CERN T9 beam line.
For this tests the HARP TPC field cage has been used with mounted on it the first version of resistive MicroMega (MM-0). The goal for these tests being the characterisation of the response of the MM-0. 

A number of samples of data have been taken under different conditions of the beam (particle types and momentum) and also of the detector working conditions. The response to muons, electrons, pions and protons at different momentum but also entering in the TPC active volume at several drift distances has been studied. Both high voltage bias and sampling time of the MM has been varied have been varied during the data taking to study the response of the detector at different working points.  Cosmic ray events  have been also recorded to study the MM response with respect to different track orientations. Finally a radioactive source of $^{55}$Fe have been positioned at the cathode to have a reference point for  energy calibration. 

In this section we present a detailed description of the experimental setup (see Section~\ref{sec:testbeam_setup}) used for the test beam as well as preliminary results obtained from a first analysis of the collected data (see Section~\ref{sec:testbeam_res}). 



\subsection{The setup}
\label{sec:testbeam_setup}

A cylindrical volume of 2~m long and $\sim$~0.8~m diameter host the drift volume. The field cage is made by Stesalit  with a double interleaved strip pattern to avoid electric field
inhomogeneities and high field gradients.
A foil of individual aluminized Mylar strips has been glued inside
the cylinder, and an aluminium foil has been glued onto the
outside surface.
A detailed description of the HARP field cage can be found in~\cite{HARP_fieldcage}.
The cathode is at one extremity of the filed cage and at about 50~cm from the edge of the external cylinder. 
Made of xxx it host on its rear holes to host calibration sources. During the TPC operation a voltage of 25 kVolts have been applied to the cathode generating an electric field in the drift volume of 167~V/cm.  
On the extremity opposite to the cathode a circular flange close the cylinder where the Micromegas MM-0 is installed. The description of the MM-0 and of the readout electronics has been detailed in Section~\ref{sec:MM}  \todo{shall we describe here the electronics?}. 

The TPC has been operated using a premixed gas with 95\% Ar , 3\% CF4 and 2\% Isobutane, which is the same mixing used by T2K for the existing ND280 TPCs. 
A simple gas system with only one line has been set up to operate the detector. Before starting the data taking the TPC has been extensively fluxed with Nitrogen gas first. Later it has been flushed with the gas mixture for several hours (3 or 4 times the volume of the TPC) to remove impurities. During normal operations the gas flux was kept of about 25 litres/hours.    Temperature measurement on the exhaust line were taken to monitor environmental condition which might induce a difference in the electron drift velocity and thus on the performances of the detector.  

To trigger on cosmic rays going through the TPC two scintillator plastic panels have been positioned on the top and the bottom of the TPC. Panels are made of 3 200(L)x20(W)x2(H) cm$^3$ bars of Polystyrene doped with 2\% PTP and 0.05\% POPOP. The surface is coated with reflective paint and two grooves are made to host fibres. The readout is done at one side with Hamamatsu MPPC while the other end-side of the fibres is mirroed. Plastic bars are installed inside aluminum boxes to get good light tightness conditions\footnote{The cosmic ray system has been kindly provided by the Neutrino Platform and the design comes from R\&D for the ICARUS cosmic ray tagger.}.  


Figure~\ref{fig:setup_tpc} shows the experimental setup during the data taking in T9. The beam is entering from the left of the picture. As previously mentioned, data were taken with the beam entering at a number of distances from the anode to test different drift distances (e.g. 30, 75 and 115 cm? ). To facilitate the displacement, the setup has been positioned on a table equipped with wheels.   




\begin{figure}[htbp]
\centering
\includegraphics[width=.7\linewidth]{TPCtestbeam_setup.png}
\caption{\label{fig:setup_tpc} The experimental setup during the TPC test beam in T9 at CERN. The Micromegas MM-0 is mounted on the HARP field cage. Two alluminium boxes containing plastic scintillator bars read out by SiPM are positioned on the top and the bottom of the field cage in order to select through going cosmic rays. }
\end{figure}





\subsubsection{The DAQ}



\subsubsection{The trigger}

Test beam data were taken using the T9 beamline with copper target to have an \" hadron enriched  beam configuration\". The breakdown of the beam composition as a function of the energy is shown in Figure~\ref{fig:T9beam}. The beam composition at low energies is largely dominated by electrons. The use of copper target allow to reduce the electron contribution of about a factor 8. \todo{I did not manage to find the same plots for the hadron enriched beams}   

\begin{figure}
\centering
\begin{subfigure}{.40\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{T9beam_positive.png}
  \caption{ \label{fig:BeamPos} }
\end{subfigure}%
\hspace{.2cm}
\begin{subfigure}{.40\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{T9beam_negative.png}
  \caption{\label{fig:BeamNeg} }
  \end{subfigure}
\caption{\label{fig:T9beam} Breakdown of the beam composition as a function of the energy for T9 for electron enriched beams. The electron composition during hadron enriched  beam configuration is strongly reduced (of about a factor 8)   }
\end{figure}



Particles coming from the beam have been tagged using three plastic scintillator detectors coupled with PMTs called respectively S1, S2, S3\footnote{The numbering of the detectors always start from the most upstream.} and two Cherenkov detectors called C1 and C2. 
Figure~\ref{fig:trigger} shows a cartoon of the locations for those detectors along the beamline.   
The selection for the different particle types have been done by the combination of the NIM signals coming from those detectors. A summary of the different options is presented in Table~\ref{tab:triggermenu}.  



\begin{figure}
\centering
\includegraphics[width=.7\linewidth]{Trigger_setup.png}
\caption{\label{fig:trigger} Cartoon of the detectors used to tag the particles from the beam and set up trigger selections.  }
\end{figure}



\begin{table}[htbp]
\centering
\begin{tabular}{l  l }
\hline
\hline

Particle  & Selection \\
\hline
Electrons & Scintillators + Cherenkov    \\
Protons (+Kaons) & S1(delayed) * S2 (delay ~ proton TOF between S1 and S2)   \\
Pions (+ muons) & Scintillators * $\overline{\mathrm{protons}}$ * $\overline{\mathrm{electrons}}$ \\ 
Cosmic ray &  from the scintillators panels (only out of spill) \\ 
\hline
\hline
\end{tabular}
\caption{\label{tab:triggermenu} Summary of the different signal combinations to tag the different particle types coming from the beam}
\end{table}


\emph{Gianmaria can possibly comment more about trigger rates.. }




\subsection{Test beam data analysis}
The main goal of this section is to present some results obtained with the data collected during TPC test beam to discuss the performance of the new resistive MM and evaluate the potential improvement of their usage in the HA-TPCs in contrast of the currently used MM installed in the forward TPCs of the ND280 detector.
\label{sec:testbeam_res}
\subsubsection{Tracks selection}
Reconstruction methods to select tracks are still under development. Since the selection of the tracks for the analysis is a critical factor the present results are still preliminary and therefore all the values provided in this section offer at most a lower bound of the future potential of resistive MM. The selection of tracks has been made using DBSCAN algorithm \todo{ref}. It allows to separate and select tracks in events with high density of triggered pads, as shown in Figure ~\ref{fig:3d_sel}, with low noise and with high acceptance allowing to perform analysis with clean and large subsets of selected data. A intuitive view of the selection is also offered in Figure ~\ref{fig:sel} where the outcome of the selection is shown projected in the read-out plane.
\iffalse 
The selection that has been used is based on the following algorithm:
\begin{itemize}
    \item select the charge clusters in the first and in the last column
    \item consider all the possible combinations between the start and end clusters as a track candidates
    \item connect start and end position with a line, define a tolerance in space and time and associate all the collected hits with a track candidate
    \item the track candidate that is horizontal, has no gaps and passes through all the detector will be successfully selected
\end{itemize}
An illustrative plot of the performance of this method is presented in Figure ~\ref{fig:sel}. In addition to it, another selection method based on DBSCAN algorithm (include reference) is under development. Since it works in 3D it can potentially fit better the tracks reducing the noise and increasing the statistics for future analysis, namely, about a factor 3 more statistics is collected using this selection.
So far, this method has demonstrated much better separation capability for multi-track events as shown in  Figure ~\ref{fig:3d_sel} and therefore will be further investigate to study the full potential of resistive MM separating close tracks, and analyzing particle showers events.
\fi

\begin{figure}[hbtp]
    \begin{center}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.5\linewidth]{sel1.pdf} \\ a) }
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.5\linewidth]{sel2.pdf} \\ b) }
    \end{minipage}
    \caption{Views of the projection of the raw event a) and one of the selected tracks b) on the read-out plane of the MM. The colormap shows the charge deposited in each pad in arbitrary units.}
    \label{fig:sel}
    \end{center}
\end{figure}
\begin{figure}[hbtp]
    \begin{center}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.99\linewidth]{multitrack1.pdf} \\ a) }
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.99\linewidth]{mutlitrack4.pdf} \\ b) }
    \end{minipage}
    \caption{Views of two events a) and b) before (left) and after (right) the selection.}
    \label{fig:3d_sel}
    \end{center}
\end{figure}

\subsubsection{dE/dx}
\begin{figure}[hbtp]
    \begin{center}
    \includegraphics[width=1.\linewidth]{dedx.pdf}
    \hspace{0.16\linewidth} a) \hspace{0.33\linewidth} b) \hspace{0.33\linewidth} c) 
    \caption{The prototype dE/dx measurements for different values of the drift distance: (a) 80 cm, (b) 30 cm, (c) 10 cm. The rows corresponds to the proton, electron and pion triggers respectively.}
    \label{fig:text_beam_dedx}
    \end{center}
\end{figure}
The preliminary studies of the dE/dx were performed with the collected data. The goal was to analyze the measured ionization loss by the different particles selected by the triggers and estimate the dE/dx resolution. For this purpose the simple selection was developed to extract beam tracks. The challenge was to suppress cosmic events, source signal and pileuped beam tracks. 
After applying the selection we extract a single beam track for the analysis. The dE/dx study was done in the most common way for the TPCs~\cite{allison1980relativistic}:
\begin{itemize}
    \item pads in the column were summarized into cluster
    \item charge in the cluster was sorted in the increasing order
    \item the clusters with the highest energy (30\% of all) were rejected
\end{itemize}
Thus we obtained nearly Gaussian distributions that describes the energy loss of the charged particles in the TPC prototype. The dE/dx distribution for various particle samples separated by the trigger are presented on the figure~\ref{fig:text_beam_dedx}.
The comparison with the current T2K TPCs dE/dx resolution is reasonable as we should be sure that the particle identification will not be worse with the new detectors. Taking into account the 2 times bigger size of the T2K TPCs (2 MM with 36 pads each) we can conclude that the measured energy resolution is nearly the same value as we observed in the ongoing experiment.
\subsubsection{Point resolution}
\par A point resolution study has been done in order to estimate the potential improvement of using resistive MM, see section~\ref{sec:MM}. In this analysis the approach in section 6.1.1 from Janssen (2008) has been followed. It is important to remark that the results are still preliminary since clusters with 4 or more pads have not been considered in the analysis. In addition the beam test data was collected with MM-0 instead of the final version MM-1, to be mounted in the final HA-TPCs. 
\begin{figure}[hbtp]
        \centering{\includegraphics[width=0.99\linewidth]{point_res.pdf} \\ a) }
    \caption{Spatial resolution of MM-0 as a function of distance for different particle beams of momentum 0.8 GeV/c.}
    \label{fig:point_res}
\end{figure}
\iffalse 
Therefore, the future results are expected to improve the preliminary values in Table~\ref{tab:point_res}
\begin{table}[hbtp]
    \centering
    \begin{tabular}{cccccc}
        \hline\hline
        Trigger & Mom [GeV/$c^2$]  & Sel. evts & dist. to MM & $\sigma_{res}$ unc. [$\mu$m] & $\sigma_{res}$ corr. [$\mu$m]   \\
        \hline
        Electrons & 0.8 & 10000 & A  & n1\\
        Electrons & 0.8 & 10000 & B  & n2\\
        Electrons & 0.8 & 10000 & C  & n3\\
        Electrons & 0.8 & 10000 & D  & n4\\
        \hline\hline
    \end{tabular}
    \caption{Preliminary point resolutions for different runs collected during the TPC test beam as a function of the Beam Momentum (Mom), number of selected events (Sel. evts) and distance to read-out plane (dist. to MM). The values of the point resolution are offered before ($\sigma_{res}$ unc.) and after ($\sigma_{res}$ corr.) applying pad response function correction. }
    \label{tab:point_res}
\end{table}
\fi
\par Using a resistive MM has the advantage of increase the average number of hit pads per event due to the charge spreading in the read-out plane. Accordingly, the study of the pad response function (PRF) may help improving the resolution if it is used to correct the input data. Assuming as true information the extrapolation of a linear fit at the cluster position and as reconstructed information the mean of the charge distribution in the same cluster it is possible to obtain the PRF information. The method followed classifies the information depending on the number of clusters since the bias in the true position it is highly correlated with the number of triggered pads in one cluster, as can be seen in Figure \ref{fig:PRF_pads}
\begin{figure}[hbtp]
    \begin{center}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{PRF_2pad.pdf} \\ a) }
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{PRF_3pad.pdf} \\ b) }
    \end{minipage}
    \caption{a) PRF for clusters with 2 pads b) PRF for clusters with 3 pads.}
    \label{fig:iron_sel}
    \end{center}
\end{figure}
\par To fully understand the behaviour of MM-0 the spatial resolution has been computed for each one of the columns of the read-out plane. As it clear in Figure \ref{fig:res_column} there are important border effects due to electric field distortions in the edges of the MM and because the charge spreading in the borders can not be read out by neighbor pads. Accordingly the values in \ref{fig:PRF_pads} do not include the values of the first and last clusters.
\begin{figure}[hbtp]
    \begin{center}
    \begin{minipage}{0.32\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{sigma_all_merged1.eps} \\ a) }
    \end{minipage}
    \begin{minipage}{0.32\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{sigma_all_merged2.eps} \\ b) }
    \end{minipage}
    \begin{minipage}{0.32\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{sigma_all_merged3.eps} \\ c) }
    \end{minipage}
    \caption{Spatial resolution of each MM column using 0.8 GeV/c momentum beam at 80cm distance for: a) Pions b) Electrons c) Protons.}
    \label{fig:res_column}
    \end{center}
\end{figure}
\par It is worth noting that even if the point resolution studies are still under development and can be fairly considered as preliminaries the values in Figure ~\ref{fig:point_res} already supersede the ones achieved by the current ND280's MM \todo{\cite{????}} showing the potential power of resistive MM.
\subsubsection{Gain studies}
An $55^$Fe radioactive source with a typical emission of 6KeV was placed in the cathode of the HARP TPC chamber during data collection. A dedicated selection to look for isolated clusters was developed to select signal charge coming from argon ionized by one $55^$Fe X-ray photon. The results of such selection are exemplified in Figure ~\ref{fig:iron_sel} 
\begin{figure}[hbtp]
    \begin{center}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{iron_before.pdf} \\ a) }
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{iron_after.pdf} \\ b) }
    \end{minipage}
    \\
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{iron_spectrum.pdf} \\ c) }
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering{\includegraphics[width=0.95\linewidth]{gain_plot.pdf} \\ d) }
    \end{minipage}
    \caption{a) View of one raw event b) Selected subsample from the raw event in \textit{a)} used for the analysis c) Iron source energy spectrum in arbitrary units d) Computed gain of the MM from the observed $55^$Fe energy spectrum at different HV.}
    \label{fig:iron_sel}
    \end{center}
\end{figure}



==> t2k2-authorlist4tdr.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% T2K2 proposal author list (for TDRs)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\INSTFE}{\affiliation{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}}
\newcommand{\INSTD}{\affiliation{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}}
\newcommand{\INSTGA}{\affiliation{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}}
\newcommand{\INSTI}{\affiliation{IRFU, CEA Saclay, Gif-sur-Yvette, France}}
\newcommand{\INSTGB}{\affiliation{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}}
\newcommand{\INSTFG}{\affiliation{Colorado State University, Department of Physics, Fort Collins, Colorado, U.S.A.}}
\newcommand{\INSTFH}{\affiliation{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}}
\newcommand{\INSTBA}{\affiliation{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France }}
\newcommand{\INSTEG}{\affiliation{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}}
\newcommand{\INSTDG}{\affiliation{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}}
\newcommand{\INSTCB}{\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}}
\newcommand{\INSTED}{\affiliation{Institut de Fisica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}}
\newcommand{\INSTEC}{\affiliation{IFIC (CSIC \& University of Valencia), Valencia, Spain}}
\newcommand{\INSTHH}{\affiliation{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}}
\newcommand{\INSTEI}{\affiliation{Imperial College London, Department of Physics, London, United Kingdom}}
\newcommand{\INSTBG}{\affiliation{INFN Laboratori Nazionali di Legnaro LNL, Padova, Italy}}
\newcommand{\INSTGF}{\affiliation{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}}
\newcommand{\INSTBE}{\affiliation{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}}
\newcommand{\INSTBF}{\affiliation{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}}
\newcommand{\INSTBD}{\affiliation{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}}
\newcommand{\INSTEB}{\affiliation{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}}
\newcommand{\INSTHI}{\affiliation{Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}}
\newcommand{\INSTHA}{\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}}
\newcommand{\INSTCC}{\affiliation{Kobe University, Kobe, Japan}}
\newcommand{\INSTCD}{\affiliation{Kyoto University, Department of Physics, Kyoto, Japan}}
\newcommand{\INSTEJ}{\affiliation{Lancaster University, Physics Department, Lancaster, United Kingdom}}
\newcommand{\INSTFC}{\affiliation{University of Liverpool, Department of Physics, Liverpool, United Kingdom}}
\newcommand{\INSTFI}{\affiliation{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}}
\newcommand{\INSTHB}{\affiliation{Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}}
\newcommand{\INSTCE}{\affiliation{Miyagi University of Education, Department of Physics, Sendai, Japan}}
\newcommand{\INSTDF}{\affiliation{National Centre for Nuclear Research, Warsaw, Poland}}
\newcommand{\INSTFJ}{\affiliation{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}}
\newcommand{\INSTGJ}{\affiliation{Okayama University, Department of Physics, Okayama, Japan}}
\newcommand{\INSTCF}{\affiliation{Osaka City University, Department of Physics, Osaka, Japan}}
\newcommand{\INSTGG}{\affiliation{Oxford University, Department of Physics, Oxford, United Kingdom}}
\newcommand{\INSTBB}{\affiliation{UPMC, Universit\'e Paris Diderot, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}}
\newcommand{\INSTGC}{\affiliation{University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}}
\newcommand{\INSTFA}{\affiliation{Queen Mary University of London, School of Physics and Astronomy, London, United Kingdom}}
\newcommand{\INSTE}{\affiliation{University of Regina, Department of Physics, Regina, Saskatchewan, Canada}}
\newcommand{\INSTGD}{\affiliation{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}}
\newcommand{\INSTHC}{\affiliation{Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}}
\newcommand{\INSTBC}{\affiliation{RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}}
\newcommand{\INSTDA}{\affiliation{University Autonoma Madrid, Department of Theoretical Physics, Madrid, Spain}}
\newcommand{\INSTFB}{\affiliation{University of Sheffield, Department of Physics and Astronomy, Sheffield, United Kingdom}}
\newcommand{\INSTDI}{\affiliation{University of Silesia, Institute of Physics, Katowice, Poland}}
\newcommand{\INSTEH}{\affiliation{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}}
\newcommand{\INSTCH}{\affiliation{University of Tokyo, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTBJ}{\affiliation{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}}
\newcommand{\INSTCG}{\affiliation{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}}
\newcommand{\INSTHF}{\affiliation{Tokyo Institute of Technology, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTGI}{\affiliation{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTHG}{\affiliation{Tokyo University of Science, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTF}{\affiliation{University of Toronto, Department of Physics, Toronto, Ontario, Canada}}
\newcommand{\INSTB}{\affiliation{TRIUMF, Vancouver, British Columbia, Canada}}
\newcommand{\INSTDJ}{\affiliation{University of Warsaw, Faculty of Physics, Warsaw, Poland}}
\newcommand{\INSTDH}{\affiliation{Warsaw University of Technology, Institute of Radioelectronics, Warsaw, Poland}}
\newcommand{\INSTFD}{\affiliation{University of Warwick, Department of Physics, Coventry, United Kingdom}}
\newcommand{\INSTGE}{\affiliation{University of Washington, Department of Physics, Seattle, Washington, U.S.A.}}
\newcommand{\INSTGH}{\affiliation{University of Winnipeg, Department of Physics, Winnipeg, Manitoba, Canada}}
\newcommand{\INSTEA}{\affiliation{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}}
\newcommand{\INSTHE}{\affiliation{Yokohama National University, Faculty of Engineering, Yokohama, Japan}}
\newcommand{\INSTH}{\affiliation{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}}
\newcommand{\INSTCERN}{\affiliation{CERN, Geneva, Switzerland}}


\INSTFE
\INSTGA
\INSTI
\INSTGB
\INSTFG
\INSTFH
\INSTBA
\INSTEG
\INSTDG
\INSTCB
\INSTED
\INSTEC
\INSTEI
\INSTBG
\INSTGF
\INSTBE
\INSTBF
\INSTBD
\INSTEB
\INSTHA
\INSTCC
\INSTCD
\INSTEJ
\INSTFC
\INSTFI
\INSTHB
\INSTCE
\INSTDF
\INSTFJ
\INSTGJ
\INSTCF
\INSTGG
\INSTBB
\INSTGC
\INSTFA
\INSTE
\INSTGD
\INSTHC
\INSTBC
\INSTDA
\INSTFB
\INSTDI
\INSTEH
\INSTCH
\INSTBJ
\INSTCG
\INSTHF
\INSTGI
\INSTHG
\INSTF
\INSTB
%\INSTG
\INSTDJ
\INSTDH
\INSTFD
\INSTGE
\INSTGH
\INSTEA
\INSTHE
\INSTH
\INSTCERN

\author{K.\,Abe}\INSTBJ
\author{H.\,Aihara}\INSTCH\INSTHA
\author{A.\,Ajmi}\INSTBF
\author{C.\,Andreopoulos}\INSTEH\INSTFC
\author{M.\,Antonova}\INSTEB
\author{S.\,Aoki}\INSTCC
\author{Y.\,Asada}\INSTHE
\author{Y.\,Ashida}\INSTCD
\author{A.\,Atherton}\INSTEH
\author{E.\,Atkin}\INSTEI
\author{D.\,Atti\'e}\INSTI
\author{S.\,Ban}\INSTCD
\author{F.C.T.\,Barbato}\INSTBE
\author{M.\,Barbi}\INSTE
\author{G.J.\,Barker}\INSTFD
\author{G.\,Barr}\INSTGG
\author{M.\,Batkiewicz}\INSTDG
\author{A.\,Beloshapkin}\INSTEB
\author{V.\,Berardi}\INSTGF
\author{L.\,Berns}\INSTHF
\author{S.\,Bhadra}\INSTH
\author{J.\,Bian}\INSTGA
\author{S.\,Bienstock}\INSTBB
\author{A.\,Blondel}\INSTEG
\author{J.\,Boix}\INSTED
\author{S.\,Bolognesi}\INSTI
\author{J.\,Borg}\INSTEI
\author{S.\,Bordoni }\INSTCERN
\author{B.\,Bourguille }\INSTED
\author{S.B.\,Boyd}\INSTFD
\author{D.\,Brailsford}\INSTEJ
\author{A.\,Bravar}\INSTEG
\author{C.\,Bronner}\INSTBJ
\author{D.\,Browning}\INSTFI
\author{M.\,Buizza Avanzini}\INSTBA
\author{F.\,Cadoux}\INSTEG
\author{N.F.\,Calabria}\INSTGF
\author{J.\,Calcutt}\INSTHB
\author{R.G.\,Calland}\INSTHA
\author{D.\,Calvet}\INSTI
\author{T.\,Campbell}\INSTFG
\author{S.\,Cao}\INSTCB
\author{S.L.\,Cartwright}\INSTFB
\author{R.\,Castillo}\INSTED
\author{M.G.\,Catanesi}\INSTGF
\author{W.\,Ceria}\INSTBB
\author{A.\,Cervera}\INSTEC
\author{A.\,Chappell}\INSTFD
\author{D.\,Cherdack}\INSTFG
\author{N.\,Chikuma}\INSTCH
\author{G.\,Christodoulou}\INSTFC
\author{M.\,Cicerchia}\INSTBG
\author{A.\,Clifton}\INSTFG
\author{G.\,Cogo}\INSTBF
\author{P.\,Colas}\INSTI
\author{J.\,Coleman}\INSTFC
\author{G.\,Collazuol}\INSTBF
\author{D.\,Coplowe}\INSTGG
\author{A.\,Cudd}\INSTHB
\author{A.\,Dabrowska}\INSTDG
\author{A.\,Delbart}\INSTI
\author{A.\,De Roeck}\INSTCERN
\author{G.\,De Rosa}\INSTBE
\author{T.\,Dealtry}\INSTEJ
\author{P.F.\,Denner}\INSTFD
\author{S.R.\,Dennis}\INSTFC
\author{C.\,Densham}\INSTEH
\author{R.\,de Oliveira}\INSTCERN
\author{D.\,Dewhurst}\INSTGG
\author{F.\,Di Lodovico}\INSTFA
\author{N.\,Dokania}\INSTFJ
\author{S.\,Dolan}\INSTGG
\author{D.\,Douqa}\INSTEG
\author{O.\,Drapier}\INSTBA
\author{K.E.\,Duffy}\INSTGG
\author{J.\,Dumarchez}\INSTBB
\author{P.J.\,Dunne}\INSTEI
\author{M.\,Dziewiecki}\INSTDH
\author{S.\,Emery-Schrenk}\INSTI
\author{A.\,Evangelisti}\INSTBE
\author{Y.\,Favre}\INSTEG
\author{S.\,Fedotov}\INSTEB
\author{P.\,Fernandez}\INSTDA
\author{T.\,Feusels}\INSTD
\author{A.J.\,Finch}\INSTEJ
\author{G.A.\,Fiorentini}\INSTH
\author{G.\,Fiorillo}\INSTBE
\author{M.\,Fitton}\INSTEH
\author{M.\,Friend}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Fujii}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{R.\,Fujita}\INSTCH
\author{D.\,Fukuda}\INSTGJ
\author{R.\,Fukuda}\INSTHG
\author{Y.\,Fukuda}\INSTCE
\author{A.\,Garcia}\INSTED
\author{C.\,Giganti}\INSTBB
\author{F.\,Gizzarelli}\INSTI
\author{M.\,Gonin}\INSTBA
\author{A.\,Gorin}\INSTEB
author{F.\,Gramegna}\INSTBG
\author{M.\,Guida}\INSTCERN
\author{M.\,Guigue}\INSTBB
\author{D.R.\,Hadley}\INSTFD
\author{L.\,Haegel}\INSTEG
\author{J.T.\,Haigh}\INSTFD
\author{P.\,Hamacher-Baumann}\INSTBC
\author{D.\,Hansen}\INSTGC
\author{J.\,Harada}\INSTCF
\author{M.\,Hartz}\INSTHA\INSTB
\author{T.\,Hasegawa}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{N.C.\,Hastings}\INSTE
\author{Y.\,Hayato}\INSTBJ\INSTHA
\author{A.\,Hiramoto}\INSTCD
\author{M.\,Hogan}\INSTFG
\author{R.\,Howell}\INSTGD
\author{J.\,Holeczek}\INSTDI
\author{F.\,Iacob}\INSTBF
\author{A.K.\,Ichikawa}\INSTCD
\author{M.\,Ikeda}\INSTBJ
\author{J.\,Imber}\INSTBA
\author{R.A.\,Intonti}\INSTGF
\author{T.\,Ishida}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{T.\,Ishii}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{T.\,Ishii}\INSTCH
\author{M.\,Ishitsuka}\INSTHG
\author{E.\,Iwai}\INSTCB
\author{K.\,Iwamoto}\INSTCH
\author{A.\,Izmaylov}\INSTEC\INSTEB
\author{B.\,Jamieson}\INSTGH
\author{C.\,Jesus-Valls}\INSTED
\author{M.\,Jiang}\INSTCD
\author{S.\,Johnson}\INSTGB
\author{J.H.\,Jo}\INSTFJ
\author{P.\,Jonsson}\INSTEI
\author{C.K.\,Jung}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFJ
\author{M.\,Kabirnezhad}\INSTDF
\author{A.C.\,Kaboth}\INSTHC\INSTEH
\author{T.\,Kajita}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTCG
\author{H.\,Kakuno}\INSTGI
\author{J.\,Kameda}\INSTBJ
\author{S.\,Kasetti}\INSTFI
\author{Y.\,Kataoka}\INSTBJ
\author{T.\,Katori}\INSTFA
\author{E.\,Kearns}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFE\INSTHA
\author{M.\,Khabibullin}\INSTEB
\author{A.\,Khotjantsev}\INSTEB
\author{T.\,Kikawa}\INSTCD
\author{H.\,Kim}\INSTCF
\author{S.\,King}\INSTFA
\author{J.\,Kisiel}\INSTDI
\author{A.\,Knight}\INSTFD
\author{A.\,Knox}\INSTEJ
\author{T.\,Kobayashi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{L.\,Koch}\INSTBC
\author{A.\,Konaka}\INSTB
\author{L.L.\,Kormos}\INSTEJ
\author{A.\,Korzenev}\INSTEG
\author{U.\,Kose}\INSTCERN
\author{A.\,Kostin}\INSTEB
\author{Y.\,Koshio}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTGJ
\author{K.\,Kowalik}\INSTDF
\author{W.\,Kropp}\INSTGA
\author{Y.\,Kudenko}\thanks{also at National Research Nuclear University "MEPhI" and Moscow Institute of Physics and Technology, Moscow, Russia}\INSTEB
\author{S.\,Kuribayashi}\INSTCD
\author{R.\,Kurjata}\INSTDH
\author{T.\,Kutter}\INSTFI
\author{M.\,Kuze}\INSTHF
\author{L.\,Labarga}\INSTDA
\author{J.\,Lagoda}\INSTDF
\author{I.\,Lamont}\INSTEJ
\author{M.\,Lamoureux}\INSTI
\author{M.\,Laveder}\INSTBF
\author{M.\,Lawe}\INSTEJ
\author{T.\,Lindner}\INSTB
\author{Z.J.\,Liptak}\INSTGB
\author{R.P.\,Litchfield}\INSTEI
\author{X.\,Li}\INSTFJ
\author{S.\,Liu}\INSTFJ
\author{K.R.\,Long}\INSTEI
\author{A.\,Longhin}\INSTBF
\author{J.P.\,Lopez}\INSTGB
\author{L.\,Ludovici}\INSTBD
\author{X.\,Lu}\INSTGG
\author{T.\,Lux}\INSTED
\author{L.\,Magaletti}\INSTGF
\author{L.\,Magro}\INSTBJ
\author{K.\,Mahn}\INSTHB
\author{M.\,Malek}\INSTFB
\author{S.\,Manly}\INSTGD
\author{T.\,Marchi}\INSTBG
\author{L.\,Maret}\INSTEG
\author{A.D.\,Marino}\INSTGB
\author{J.F.\,Martin}\INSTF
\author{S.\,Martynenko}\INSTFJ
\author{T.\,Maruyama}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{J.\,Marzec}\INSTDH
\author{T.\,Matsubara}\INSTCB
\author{K.\,Matsushita}\INSTCH
\author{V.\,Matveev}\INSTEB
\author{K.\,Mavrokoridis}\INSTFC
\author{E.\,Mazzucato}\INSTI
\author{M.\,McCarthy}\INSTH
\author{N.\,McCauley}\INSTFC
\author{K.S.\,McFarland}\INSTGD
\author{C.\,McGrew}\INSTFJ
\author{A.\,Mefodiev}\INSTEB
\author{B.\,Mehl}\INSTCERN
\author{P.\,Mermod}\INSTEG
\author{C.\,Metelko}\INSTFC
\author{M.\,Mezzetto}\INSTBF
\author{J.\,Michalowski}\INSTDG
\author{P.\,Mijakowski}\INSTDF
\author{A.\,Minamino}\INSTHE
\author{O.\,Mineev}\INSTEB
\author{S.\,Mine}\INSTGA
\author{A.\,Missert}\INSTGB
\author{M.\,Miura}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{D.\,Mladenov}\INSTCERN
\author{S.\,Monsalvo}\INSTCERN
\author{S.\,Moriyama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{J.\,Morrison}\INSTHB
\author{Th.A.\,Mueller}\INSTBA
\author{J.\,Mundet}\INSTED
\author{Y.\,Nagai}\INSTGB
\author{T.\,Nakadaira}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Nakahata}\INSTBJ\INSTHA
\author{Y.\,Nakajima}\INSTBJ
\author{A.\,Nakamura}\INSTGJ
\author{K.G.\,Nakamura}\INSTCD
\author{K.\,Nakamura}\thanks{also at J-PARC, Tokai, Japan}\INSTHA\INSTCB
\author{S.\,Nakayama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{T.\,Nakaya}\INSTCD\INSTHA
\author{K.\,Nakayoshi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{C.\,Nantais}\INSTF
\author{L.\,Nascimento Machado}\INSTBE
\author{M.\,Nessi}\INSTCERN
\author{T.V.\,Ngoc}\INSTHH
\author{K.\,Nishikawa}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Nishimura}\INSTCG
\author{E.\,Noah}\INSTEG
\author{T.\,Nonnenmacher}\INSTEI
\author{P.\,Novella}\INSTEC
\author{J.\,Nowak}\INSTEJ
\author{H.M.\,O'Keeffe}\INSTEJ
\author{T.\,Odagawa}\INSTCD
\author{R.\,Ohta}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{K.\,Okamoto}\INSTHE
\author{K.\,Okumura}\INSTCG\INSTHA
\author{T.\,Okusawa}\INSTCF
\author{Y.\,Orain}\INSTBB
\author{T.\,Ovsyannikova}\INSTEB
\author{R.A.\,Owen}\INSTFA
\author{Y.\,Oyama}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{V.\,Palladino}\INSTBE
\author{J.L.\,Palomino}\INSTFJ
\author{V.\,Paolone}\INSTGC
\author{J.M.\,Parraud}\INSTBB
\author{M.\,Pari}\INSTBF
\author{W.\,Parker}\INSTHC
\author{S.\,Parsa}\INSTEG
\author{J.\,Pasternak}\INSTEI
\author{C.\,Pastore}\INSTGF
\author{M.\,Pavin}\INSTBB
\author{D.\,Payne}\INSTFC
\author{A.\,Pepato}\INSTBF
\author{J.D.\,Perkin}\INSTFB
\author{F.\,Pietropaolo}\INSTCERN
\author{L.\,Pickard}\INSTFB
\author{L.\,Pickering}\INSTHB
\author{E.S.\,Pinzon Guerra}\INSTH
\author{O.\,Pizzirusso}\INSTCERN
\author{B.\,Popov}\thanks{also at JINR, Dubna, Russia}\INSTBB
\author{J.\,Porthault}\INSTI
\author{M.\,Posiadala-Zezula}\INSTDJ
\author{J.-M.\,Poutissou}\INSTB
\author{R.\,Poutissou}\INSTB
\author{J.\,Pozimski}\INSTEI
\author{P.\,Przewlocki}\INSTDF
\author{H.\,Przybilski}\INSTDG
\author{B.\,Quilain}\INSTCB
\author{T.\,Radermacher}\INSTBC
\author{E.\,Radicioni}\INSTGF
\author{P.N.\,Ratoff}\INSTEJ
\author{M.\,Ravonel}\INSTEG
\author{M.A.M.\,Rayner}\INSTEG
\author{E.\,Reinherz-Aronis}\INSTFG
\author{F.\,Resnati}\INSTCERN
\author{M.\,Riallot}\INSTI
\author{C.\,Riccio}\INSTBE
\author{P.\,Rojas}\INSTFG
\author{G.\,Romanino}\INSTBF
\author{E.\,Rondio}\INSTDF
\author{B.\,Rossi}\INSTBE
\author{F.\,Rossi}\INSTI
\author{S.\,Roth}\INSTBC
\author{A.C.\,Ruggeri}\INSTBE
\author{A.\,Rychter}\INSTDH
\author{K.\,Sakashita}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{F.\,S\'anchez}\INSTEG
\author{E.\,Scantamburlo}\INSTEG
\author{K.\,Scholberg}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFH
\author{J.\,Schwehr}\INSTFG
\author{M.\,Scott}\INSTEI
\author{Y.\,Seiya}\INSTCF
\author{T.\,Sekiguchi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{H.\,Sekiya}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ\INSTHA
\author{D.\,Sgalaberna}\INSTEG
\author{A.\,Shaikina}\INSTEB
\author{R.\,Shah}\INSTEH\INSTGG
\author{A.\,Shaikhiev}\INSTEB
\author{F.\,Shaker}\INSTGH
\author{D.\,Shaw}\INSTEJ
\author{M.\,Shiozawa}\INSTBJ\INSTHA
\author{T.\,Shirahige}\INSTGJ
\author{W.\,Shorrock}\INSTEI
\author{A.\,Smirnov}\INSTEB
\author{M.\,Smy}\INSTGA
\author{J.T.\,Sobczyk}\INSTEA
\author{H.\,Sobel}\INSTGA\INSTHA
\author{L.\,Southwell}\INSTEJ
\author{R.\,Spina}\INSTGF
\author{J.\,Steinmann}\INSTBC
\author{T.\,Stewart}\INSTEH
\author{P.\,Stowell}\INSTFB
\author{S.\,Suvorov}\INSTEB
\author{A.\,Suzuki}\INSTCC
\author{S.Y.\,Suzuki}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Suzuki}\INSTHA
\author{M.\,Szeptycka}\INSTDF
\author{S.\,Szoldos}\INSTFA
\author{A.\,Sztuc}\INSTEI
\author{J.\,Swierblewski}\INSTDG
\author{R.\,Tacik}\INSTE\INSTB
\author{M.\,Tada}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Tajima}\INSTCD
\author{A.\,Takeda}\INSTBJ
\author{Y.\,Takeuchi}\INSTCC\INSTHA
\author{H.K.\,Tanaka}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{H.A.\,Tanaka}\thanks{also at Institute of Particle Physics, Canada}\INSTF\INSTB
\author{A.\,Teklu}\INSTFJ
\author{D.\,Terhorst}\INSTBC
\author{L.F.\,Thompson}\INSTFB
\author{W.\,Toki}\INSTFG
\author{T.\,Tomura}\INSTBJ
\author{C.\,Touramanis}\INSTFC
\author{T.\,Tsukamoto}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Tzanov}\INSTFI
\author{M.A.\,Uchida}\INSTEI
\author{Y.\,Uchida}\INSTEI
\author{M.\,Vagins}\INSTHA\INSTGA
\author{Z.\,Vallari}\INSTFJ
\author{N.H.\,Van}\INSTHH\INSTHI
\author{D.\,Vargas}\INSTED
\author{G.\,Vasseur}\INSTI
\author{T.\,Wachala}\INSTDG
\author{C.W.\,Walter}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFH
\author{D.\,Wark}\INSTEH\INSTGG
\author{M.O.\,Wascko}\INSTEI
\author{A.\,Weber}\INSTEH\INSTGG
\author{R.\,Wendell}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTCD
\author{L.\,Whitehead}\INSTCERN
\author{R.J.\,Wilkes}\INSTGE
\author{M.J.\,Wilking}\INSTFJ
\author{J.R.\,Wilson}\INSTFA
\author{R.J.\,Wilson}\INSTFG
\author{C.\,Wret}\INSTGD
\author{Y.\,Yamada}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{K.\,Yamamoto}\INSTCF
\author{C.\,Yanagisawa}\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}\INSTFJ
\author{G.\,Yang}\INSTFJ
\author{T.\,Yano}\INSTBJ
\author{K.\,Yasutome}\INSTCD
\author{S.\,Yen}\INSTB
\author{N.\,Yershov}\INSTEB
\author{M.\,Yokoyama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTCH
\author{T.\,Yoshida}\INSTHF
\author{T.\,Yuan}\INSTGB
\author{M.\,Yu}\INSTH
\author{A.\,Zalewska}\INSTDG
\author{J.\,Zalipska}\INSTDF
\author{L.\,Zambelli}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{K.\,Zaremba}\INSTDH
\author{M.\,Ziembicki}\INSTDH
\author{P.\,Zilberman}\INSTFJ
\author{E.D.\,Zimmerman}\INSTGB
\author{M.\,Zito}\INSTI

\collaboration{The T2K Collaboration}\noaffiliation


==> t2k2-authorlist4tdr_mod-MZ.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% T2K2 proposal author list (for TDRs)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\INSTFE}{\affiliation{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}}
\newcommand{\INSTD}{\affiliation{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}}
\newcommand{\INSTGA}{\affiliation{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}}
\newcommand{\INSTI}{\affiliation{IRFU, CEA Saclay, Gif-sur-Yvette, France}}
\newcommand{\INSTGB}{\affiliation{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}}
\newcommand{\INSTFG}{\affiliation{Colorado State University, Department of Physics, Fort Collins, Colorado, U.S.A.}}
\newcommand{\INSTFH}{\affiliation{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}}
\newcommand{\INSTBA}{\affiliation{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France }}
\newcommand{\INSTEG}{\affiliation{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}}
\newcommand{\INSTDG}{\affiliation{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}}
\newcommand{\INSTCB}{\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}}
\newcommand{\INSTED}{\affiliation{Institut de Fisica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}}
\newcommand{\INSTEC}{\affiliation{IFIC (CSIC \& University of Valencia), Valencia, Spain}}
\newcommand{\INSTHH}{\affiliation{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}}
\newcommand{\INSTEI}{\affiliation{Imperial College London, Department of Physics, London, United Kingdom}}
\newcommand{\INSTBG}{\affiliation{INFN Laboratori Nazionali di Legnaro LNL, Padova, Italy}}
\newcommand{\INSTGF}{ {INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}}
\newcommand{\INSTBE}{ {INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}}
\newcommand{\INSTBF}{ {INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}}
\newcommand{\INSTBD}{ {INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}}
\newcommand{\INSTEB}{ {Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}}
\newcommand{\INSTHI}{ {Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}}
\newcommand{\INSTHA}{ {Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}}
\newcommand{\INSTCC}{ {Kobe University, Kobe, Japan}}
\newcommand{\INSTCD}{ {Kyoto University, Department of Physics, Kyoto, Japan}}
\newcommand{\INSTEJ}{ {Lancaster University, Physics Department, Lancaster, United Kingdom}}
\newcommand{\INSTFC}{ {University of Liverpool, Department of Physics, Liverpool, United Kingdom}}
\newcommand{\INSTFI}{ {Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}}
\newcommand{\INSTHB}{ {Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}}
\newcommand{\INSTCE}{ {Miyagi University of Education, Department of Physics, Sendai, Japan}}
\newcommand{\INSTDF}{ {National Centre for Nuclear Research, Warsaw, Poland}}
\newcommand{\INSTFJ}{ {State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}}
\newcommand{\INSTGJ}{ {Okayama University, Department of Physics, Okayama, Japan}}
\newcommand{\INSTCF}{ {Osaka City University, Department of Physics, Osaka, Japan}}
\newcommand{\INSTGG}{ {Oxford University, Department of Physics, Oxford, United Kingdom}}
\newcommand{\INSTBB}{ {UPMC, Universit\'e Paris Diderot, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}}
\newcommand{\INSTGC}{ {University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}}
\newcommand{\INSTFA}{ {Queen Mary University of London, School of Physics and Astronomy, London, United Kingdom}}
\newcommand{\INSTE}{ {University of Regina, Department of Physics, Regina, Saskatchewan, Canada}}
\newcommand{\INSTGD}{ {University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}}
\newcommand{\INSTHC}{ {Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}}
\newcommand{\INSTBC}{ {RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}}
\newcommand{\INSTDA}{ {University Autonoma Madrid, Department of Theoretical Physics, Madrid, Spain}}
\newcommand{\INSTFB}{ {University of Sheffield, Department of Physics and Astronomy, Sheffield, United Kingdom}}
\newcommand{\INSTDI}{ {University of Silesia, Institute of Physics, Katowice, Poland}}
\newcommand{\INSTEH}{ {STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}}
\newcommand{\INSTCH}{ {University of Tokyo, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTBJ}{ {University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}}
\newcommand{\INSTCG}{ {University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}}
\newcommand{\INSTHF}{ {Tokyo Institute of Technology, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTGI}{ {Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTHG}{ {Tokyo University of Science, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTF}{ {University of Toronto, Department of Physics, Toronto, Ontario, Canada}}
\newcommand{\INSTB}{ {TRIUMF, Vancouver, British Columbia, Canada}}
\newcommand{\INSTDJ}{ {University of Warsaw, Faculty of Physics, Warsaw, Poland}}
\newcommand{\INSTDH}{ {Warsaw University of Technology, Institute of Radioelectronics, Warsaw, Poland}}
\newcommand{\INSTFD}{ {University of Warwick, Department of Physics, Coventry, United Kingdom}}
\newcommand{\INSTGE}{ {University of Washington, Department of Physics, Seattle, Washington, U.S.A.}}
\newcommand{\INSTGH}{ {University of Winnipeg, Department of Physics, Winnipeg, Manitoba, Canada}}
\newcommand{\INSTEA}{ {Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}}
\newcommand{\INSTHE}{ {Yokohama National University, Faculty of Engineering, Yokohama, Japan}}
\newcommand{\INSTH}{ {York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}}
\newcommand{\INSTCERN}{ {CERN, Geneva, Switzerland}}


\INSTFE
\INSTGA
\INSTI
\INSTGB
\INSTFG
\INSTFH
\INSTBA
\INSTEG
\INSTDG
\INSTCB
\INSTED
\INSTEC
\INSTEI
\INSTBG
\INSTGF
\INSTBE
\INSTBF
\INSTBD
\INSTEB
\INSTHA
\INSTCC
\INSTCD
\INSTEJ
\INSTFC
\INSTFI
\INSTHB
\INSTCE
\INSTDF
\INSTFJ
\INSTGJ
\INSTCF
\INSTGG
\INSTBB
\INSTGC
\INSTFA
\INSTE
\INSTGD
\INSTHC
\INSTBC
\INSTDA
\INSTFB
\INSTDI
\INSTEH
\INSTCH
\INSTBJ
\INSTCG
\INSTHF
\INSTGI
\INSTHG
\INSTF
\INSTB
%\INSTG
\INSTDJ
\INSTDH
\INSTFD
\INSTGE
\INSTGH
\INSTEA
\INSTHE
\INSTH
\INSTCERN

\author{K.\,Abe}\INSTBJ
\author{H.\,Aihara}\INSTCH\INSTHA
\author{A.\,Ajmi}\INSTBF
\author{C.\,Andreopoulos}\INSTEH\INSTFC
\author{M.\,Antonova}\INSTEB
\author{S.\,Aoki}\INSTCC
\author{Y.\,Asada}\INSTHE
\author{Y.\,Ashida}\INSTCD
\author{A.\,Atherton}\INSTEH
\author{E.\,Atkin}\INSTEI
\author{D.\,Atti\'e}\INSTI
\author{S.\,Ban}\INSTCD
\author{F.C.T.\,Barbato}\INSTBE
\author{M.\,Barbi}\INSTE
\author{G.J.\,Barker}\INSTFD
\author{G.\,Barr}\INSTGG
\author{M.\,Batkiewicz}\INSTDG
\author{A.\,Beloshapkin}\INSTEB
\author{V.\,Berardi}\INSTGF
\author{L.\,Berns}\INSTHF
\author{S.\,Bhadra}\INSTH
\author{J.\,Bian}\INSTGA
\author{S.\,Bienstock}\INSTBB
\author{A.\,Blondel}\INSTEG
\author{J.\,Boix}\INSTED
\author{S.\,Bolognesi}\INSTI
\author{J.\,Borg}\INSTEI
\author{S.\,Bordoni }\INSTCERN
\author{B.\,Bourguille }\INSTED
\author{S.B.\,Boyd}\INSTFD
\author{D.\,Brailsford}\INSTEJ
\author{A.\,Bravar}\INSTEG
\author{C.\,Bronner}\INSTBJ
\author{D.\,Browning}\INSTFI
\author{M.\,Buizza Avanzini}\INSTBA
\author{F.\,Cadoux}\INSTEG
\author{N.F.\,Calabria}\INSTGF
\author{J.\,Calcutt}\INSTHB
\author{R.G.\,Calland}\INSTHA
\author{D.\,Calvet}\INSTI
\author{T.\,Campbell}\INSTFG
\author{S.\,Cao}\INSTCB
\author{S.L.\,Cartwright}\INSTFB
\author{R.\,Castillo}\INSTED
\author{M.G.\,Catanesi}\INSTGF
\author{W.\,Ceria}\INSTBB
\author{A.\,Cervera}\INSTEC
\author{A.\,Chappell}\INSTFD
\author{D.\,Cherdack}\INSTFG
\author{N.\,Chikuma}\INSTCH
\author{G.\,Christodoulou}\INSTFC
\author{M.\,Cicerchia}\INSTBG
\author{A.\,Clifton}\INSTFG
\author{G.\,Cogo}\INSTBF
\author{P.\,Colas}\INSTI
\author{J.\,Coleman}\INSTFC
\author{G.\,Collazuol}\INSTBF
\author{D.\,Coplowe}\INSTGG
\author{A.\,Cudd}\INSTHB
\author{A.\,Dabrowska}\INSTDG
\author{A.\,Delbart}\INSTI
\author{A.\,De Roeck}\INSTCERN
\author{G.\,De Rosa}\INSTBE
\author{T.\,Dealtry}\INSTEJ
\author{P.F.\,Denner}\INSTFD
\author{S.R.\,Dennis}\INSTFC
\author{C.\,Densham}\INSTEH
\author{R.\,de Oliveira}\INSTCERN
\author{D.\,Dewhurst}\INSTGG
\author{F.\,Di Lodovico}\INSTFA
\author{N.\,Dokania}\INSTFJ
\author{S.\,Dolan}\INSTGG
\author{D.\,Douqa}\INSTEG
\author{O.\,Drapier}\INSTBA
\author{K.E.\,Duffy}\INSTGG
\author{J.\,Dumarchez}\INSTBB
\author{P.J.\,Dunne}\INSTEI
\author{M.\,Dziewiecki}\INSTDH
\author{S.\,Emery-Schrenk}\INSTI
\author{A.\,Evangelisti}\INSTBE
\author{Y.\,Favre}\INSTEG
\author{S.\,Fedotov}\INSTEB
\author{P.\,Fernandez}\INSTDA
\author{T.\,Feusels}\INSTD
\author{A.J.\,Finch}\INSTEJ
\author{G.A.\,Fiorentini}\INSTH
\author{G.\,Fiorillo}\INSTBE
\author{M.\,Fitton}\INSTEH
\author{M.\,Friend}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Fujii}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{R.\,Fujita}\INSTCH
\author{D.\,Fukuda}\INSTGJ
\author{R.\,Fukuda}\INSTHG
\author{Y.\,Fukuda}\INSTCE
\author{A.\,Garcia}\INSTED
\author{C.\,Giganti}\INSTBB
\author{F.\,Gizzarelli}\INSTI
\author{M.\,Gonin}\INSTBA
\author{A.\,Gorin}\INSTEB
author{F.\,Gramegna}\INSTBG
\author{M.\,Guida}\INSTCERN
\author{M.\,Guigue}\INSTBB
\author{D.R.\,Hadley}\INSTFD
\author{L.\,Haegel}\INSTEG
\author{J.T.\,Haigh}\INSTFD
\author{P.\,Hamacher-Baumann}\INSTBC
\author{D.\,Hansen}\INSTGC
\author{J.\,Harada}\INSTCF
\author{M.\,Hartz}\INSTHA\INSTB
\author{T.\,Hasegawa}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{N.C.\,Hastings}\INSTE
\author{Y.\,Hayato}\INSTBJ\INSTHA
\author{A.\,Hiramoto}\INSTCD
\author{M.\,Hogan}\INSTFG
\author{R.\,Howell}\INSTGD
\author{J.\,Holeczek}\INSTDI
\author{F.\,Iacob}\INSTBF
\author{A.K.\,Ichikawa}\INSTCD
\author{M.\,Ikeda}\INSTBJ
\author{J.\,Imber}\INSTBA
\author{R.A.\,Intonti}\INSTGF
\author{T.\,Ishida}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{T.\,Ishii}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{T.\,Ishii}\INSTCH
\author{M.\,Ishitsuka}\INSTHG
\author{E.\,Iwai}\INSTCB
\author{K.\,Iwamoto}\INSTCH
\author{A.\,Izmaylov}\INSTEC\INSTEB
\author{B.\,Jamieson}\INSTGH
\author{C.\,Jesus-Valls}\INSTED
\author{M.\,Jiang}\INSTCD
\author{S.\,Johnson}\INSTGB
\author{J.H.\,Jo}\INSTFJ
\author{P.\,Jonsson}\INSTEI
\author{C.K.\,Jung}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFJ
\author{M.\,Kabirnezhad}\INSTDF
\author{A.C.\,Kaboth}\INSTHC\INSTEH
\author{T.\,Kajita}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTCG
\author{H.\,Kakuno}\INSTGI
\author{J.\,Kameda}\INSTBJ
\author{S.\,Kasetti}\INSTFI
\author{Y.\,Kataoka}\INSTBJ
\author{T.\,Katori}\INSTFA
\author{E.\,Kearns}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFE\INSTHA
\author{M.\,Khabibullin}\INSTEB
\author{A.\,Khotjantsev}\INSTEB
\author{T.\,Kikawa}\INSTCD
\author{H.\,Kim}\INSTCF
\author{S.\,King}\INSTFA
\author{J.\,Kisiel}\INSTDI
\author{A.\,Knight}\INSTFD
\author{A.\,Knox}\INSTEJ
\author{T.\,Kobayashi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{L.\,Koch}\INSTBC
\author{A.\,Konaka}\INSTB
\author{L.L.\,Kormos}\INSTEJ
\author{A.\,Korzenev}\INSTEG
\author{U.\,Kose}\INSTCERN
\author{A.\,Kostin}\INSTEB
\author{Y.\,Koshio}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTGJ
\author{K.\,Kowalik}\INSTDF
\author{W.\,Kropp}\INSTGA
\author{Y.\,Kudenko}\thanks{also at National Research Nuclear University "MEPhI" and Moscow Institute of Physics and Technology, Moscow, Russia}\INSTEB
\author{S.\,Kuribayashi}\INSTCD
\author{R.\,Kurjata}\INSTDH
\author{T.\,Kutter}\INSTFI
\author{M.\,Kuze}\INSTHF
\author{L.\,Labarga}\INSTDA
\author{J.\,Lagoda}\INSTDF
\author{I.\,Lamont}\INSTEJ
\author{M.\,Lamoureux}\INSTI
\author{M.\,Laveder}\INSTBF
\author{M.\,Lawe}\INSTEJ
\author{T.\,Lindner}\INSTB
\author{Z.J.\,Liptak}\INSTGB
\author{R.P.\,Litchfield}\INSTEI
\author{X.\,Li}\INSTFJ
\author{S.\,Liu}\INSTFJ
\author{K.R.\,Long}\INSTEI
\author{A.\,Longhin}\INSTBF
\author{J.P.\,Lopez}\INSTGB
\author{L.\,Ludovici}\INSTBD
\author{X.\,Lu}\INSTGG
\author{T.\,Lux}\INSTED
\author{L.\,Magaletti}\INSTGF
\author{L.\,Magro}\INSTBJ
\author{K.\,Mahn}\INSTHB
\author{M.\,Malek}\INSTFB
\author{S.\,Manly}\INSTGD
\author{T.\,Marchi}\INSTBG
\author{L.\,Maret}\INSTEG
\author{A.D.\,Marino}\INSTGB
\author{J.F.\,Martin}\INSTF
\author{S.\,Martynenko}\INSTFJ
\author{T.\,Maruyama}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{J.\,Marzec}\INSTDH
\author{T.\,Matsubara}\INSTCB
\author{K.\,Matsushita}\INSTCH
\author{V.\,Matveev}\INSTEB
\author{K.\,Mavrokoridis}\INSTFC
\author{E.\,Mazzucato}\INSTI
\author{M.\,McCarthy}\INSTH
\author{N.\,McCauley}\INSTFC
\author{K.S.\,McFarland}\INSTGD
\author{C.\,McGrew}\INSTFJ
\author{A.\,Mefodiev}\INSTEB
\author{B.\,Mehl}\INSTCERN
\author{P.\,Mermod}\INSTEG
\author{C.\,Metelko}\INSTFC
\author{M.\,Mezzetto}\INSTBF
\author{J.\,Michalowski}\INSTDG
\author{P.\,Mijakowski}\INSTDF
\author{A.\,Minamino}\INSTHE
\author{O.\,Mineev}\INSTEB
\author{S.\,Mine}\INSTGA
\author{A.\,Missert}\INSTGB
\author{M.\,Miura}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{D.\,Mladenov}\INSTCERN
\author{S.\,Monsalvo}\INSTCERN
\author{S.\,Moriyama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{J.\,Morrison}\INSTHB
\author{Th.A.\,Mueller}\INSTBA
\author{J.\,Mundet}\INSTED
\author{Y.\,Nagai}\INSTGB
\author{T.\,Nakadaira}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Nakahata}\INSTBJ\INSTHA
\author{Y.\,Nakajima}\INSTBJ
\author{A.\,Nakamura}\INSTGJ
\author{K.G.\,Nakamura}\INSTCD
\author{K.\,Nakamura}\thanks{also at J-PARC, Tokai, Japan}\INSTHA\INSTCB
\author{S.\,Nakayama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{T.\,Nakaya}\INSTCD\INSTHA
\author{K.\,Nakayoshi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{C.\,Nantais}\INSTF
\author{L.\,Nascimento Machado}\INSTBE
\author{M.\,Nessi}\INSTCERN
\author{T.V.\,Ngoc}\INSTHH
\author{K.\,Nishikawa}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Nishimura}\INSTCG
\author{E.\,Noah}\INSTEG
\author{T.\,Nonnenmacher}\INSTEI
\author{P.\,Novella}\INSTEC
\author{J.\,Nowak}\INSTEJ
\author{H.M.\,O'Keeffe}\INSTEJ
\author{T.\,Odagawa}\INSTCD
\author{R.\,Ohta}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{K.\,Okamoto}\INSTHE
\author{K.\,Okumura}\INSTCG\INSTHA
\author{T.\,Okusawa}\INSTCF
\author{Y.\,Orain}\INSTBB
\author{T.\,Ovsyannikova}\INSTEB
\author{R.A.\,Owen}\INSTFA
\author{Y.\,Oyama}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{V.\,Palladino}\INSTBE
\author{J.L.\,Palomino}\INSTFJ
\author{V.\,Paolone}\INSTGC
\author{J.M.\,Parraud}\INSTBB
\author{M.\,Pari}\INSTBF
\author{W.\,Parker}\INSTHC
\author{S.\,Parsa}\INSTEG
\author{J.\,Pasternak}\INSTEI
\author{C.\,Pastore}\INSTGF
\author{M.\,Pavin}\INSTBB
\author{D.\,Payne}\INSTFC
\author{A.\,Pepato}\INSTBF
\author{J.D.\,Perkin}\INSTFB
\author{F.\,Pietropaolo}\INSTCERN
\author{L.\,Pickard}\INSTFB
\author{L.\,Pickering}\INSTHB
\author{E.S.\,Pinzon Guerra}\INSTH
\author{O.\,Pizzirusso}\INSTCERN
\author{B.\,Popov}\thanks{also at JINR, Dubna, Russia}\INSTBB
\author{J.\,Porthault}\INSTI
\author{M.\,Posiadala-Zezula}\INSTDJ
\author{J.-M.\,Poutissou}\INSTB
\author{R.\,Poutissou}\INSTB
\author{J.\,Pozimski}\INSTEI
\author{P.\,Przewlocki}\INSTDF
\author{H.\,Przybilski}\INSTDG
\author{B.\,Quilain}\INSTCB
\author{T.\,Radermacher}\INSTBC
\author{E.\,Radicioni}\INSTGF
\author{P.N.\,Ratoff}\INSTEJ
\author{M.\,Ravonel}\INSTEG
\author{M.A.M.\,Rayner}\INSTEG
\author{E.\,Reinherz-Aronis}\INSTFG
\author{F.\,Resnati}\INSTCERN
\author{M.\,Riallot}\INSTI
\author{C.\,Riccio}\INSTBE
\author{P.\,Rojas}\INSTFG
\author{G.\,Romanino}\INSTBF
\author{E.\,Rondio}\INSTDF
\author{B.\,Rossi}\INSTBE
\author{F.\,Rossi}\INSTI
\author{S.\,Roth}\INSTBC
\author{A.C.\,Ruggeri}\INSTBE
\author{A.\,Rychter}\INSTDH
\author{K.\,Sakashita}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{F.\,S\'anchez}\INSTEG
\author{E.\,Scantamburlo}\INSTEG
\author{K.\,Scholberg}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFH
\author{J.\,Schwehr}\INSTFG
\author{M.\,Scott}\INSTEI
\author{Y.\,Seiya}\INSTCF
\author{T.\,Sekiguchi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{H.\,Sekiya}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ\INSTHA
\author{D.\,Sgalaberna}\INSTEG
\author{A.\,Shaikina}\INSTEB
\author{R.\,Shah}\INSTEH\INSTGG
\author{A.\,Shaikhiev}\INSTEB
\author{F.\,Shaker}\INSTGH
\author{D.\,Shaw}\INSTEJ
\author{M.\,Shiozawa}\INSTBJ\INSTHA
\author{T.\,Shirahige}\INSTGJ
\author{W.\,Shorrock}\INSTEI
\author{A.\,Smirnov}\INSTEB
\author{M.\,Smy}\INSTGA
\author{J.T.\,Sobczyk}\INSTEA
\author{H.\,Sobel}\INSTGA\INSTHA
\author{L.\,Southwell}\INSTEJ
\author{R.\,Spina}\INSTGF
\author{J.\,Steinmann}\INSTBC
\author{T.\,Stewart}\INSTEH
\author{P.\,Stowell}\INSTFB
\author{S.\,Suvorov}\INSTEB
\author{A.\,Suzuki}\INSTCC
\author{S.Y.\,Suzuki}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Suzuki}\INSTHA
\author{M.\,Szeptycka}\INSTDF
\author{S.\,Szoldos}\INSTFA
\author{A.\,Sztuc}\INSTEI
\author{J.\,Swierblewski}\INSTDG
\author{R.\,Tacik}\INSTE\INSTB
\author{M.\,Tada}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Tajima}\INSTCD
\author{A.\,Takeda}\INSTBJ
\author{Y.\,Takeuchi}\INSTCC\INSTHA
\author{H.K.\,Tanaka}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{H.A.\,Tanaka}\thanks{also at Institute of Particle Physics, Canada}\INSTF\INSTB
\author{A.\,Teklu}\INSTFJ
\author{D.\,Terhorst}\INSTBC
\author{L.F.\,Thompson}\INSTFB
\author{W.\,Toki}\INSTFG
\author{T.\,Tomura}\INSTBJ
\author{C.\,Touramanis}\INSTFC
\author{T.\,Tsukamoto}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Tzanov}\INSTFI
\author{M.A.\,Uchida}\INSTEI
\author{Y.\,Uchida}\INSTEI
\author{M.\,Vagins}\INSTHA\INSTGA
\author{Z.\,Vallari}\INSTFJ
\author{N.H.\,Van}\INSTHH\INSTHI
\author{D.\,Vargas}\INSTED
\author{G.\,Vasseur}\INSTI
\author{T.\,Wachala}\INSTDG
\author{C.W.\,Walter}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFH
\author{D.\,Wark}\INSTEH\INSTGG
\author{M.O.\,Wascko}\INSTEI
\author{A.\,Weber}\INSTEH\INSTGG
\author{R.\,Wendell}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTCD
\author{L.\,Whitehead}\INSTCERN
\author{R.J.\,Wilkes}\INSTGE
\author{M.J.\,Wilking}\INSTFJ
\author{J.R.\,Wilson}\INSTFA
\author{R.J.\,Wilson}\INSTFG
\author{C.\,Wret}\INSTGD
\author{Y.\,Yamada}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{K.\,Yamamoto}\INSTCF
\author{C.\,Yanagisawa}\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}\INSTFJ
\author{G.\,Yang}\INSTFJ
\author{T.\,Yano}\INSTBJ
\author{K.\,Yasutome}\INSTCD
\author{S.\,Yen}\INSTB
\author{N.\,Yershov}\INSTEB
\author{M.\,Yokoyama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTCH
\author{T.\,Yoshida}\INSTHF
\author{T.\,Yuan}\INSTGB
\author{M.\,Yu}\INSTH
\author{A.\,Zalewska}\INSTDG
\author{J.\,Zalipska}\INSTDF
\author{L.\,Zambelli}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{K.\,Zaremba}\INSTDH
\author{M.\,Ziembicki}\INSTDH
\author{P.\,Zilberman}\INSTFJ
\author{E.D.\,Zimmerman}\INSTGB
\author{M.\,Zito}\INSTI

\collaboration{The T2K Collaboration}\noaffiliation

